BooookScore: A systematic exploration of book-length summarization in the era of LLMs

Summarizing book-length documents (>100K tokens) that exceed the context window size of large language models (LLMs) requires first breaking the input document into smaller chunks and then prompting an LLM to merge, update, and compress chunk-level summaries. Despite the complexity and importance of this task, it has yet to be meaningfully studied due to the challenges of evaluation: existing book-length summarization datasets (e.g., BookSum) are in the pretraining data of most public LLMs, and existing evaluation methods struggle to capture errors made by modern LLM summarizers. In this paper, we present the first study of the coherence of LLM-based book-length summarizers implemented via two prompting workflows: (1) hierarchically merging chunk-level summaries, and (2) incrementally updating a running summary. We obtain 1193 fine-grained human annotations on GPT-4 generated summaries of 100 recently-published books and identify eight common types of coherence errors made by LLMs. Because human evaluation is expensive and time-consuming, we develop an automatic metric, BooookScore, that measures the proportion of sentences in a summary that do not contain any of the identified error types. BooookScore has high agreement with human annotations and allows us to systematically evaluate the impact of many other critical parameters (e.g., chunk size, base LLM) while saving $15K USD and 500 hours in human evaluation costs. We find that closed-source LLMs such as GPT-4 and Claude 2 produce summaries with higher BooookScore than those generated by open-source models. While LLaMA 2 falls behind other models, Mixtral achieves performance on par with GPT-3.5-Turbo. Incremental updating yields lower BooookScore but higher level of detail than hierarchical merging, a trade-off sometimes preferred by annotators.

==> sections/claude.tex <==
\section{Claude experiments}

We tried incremental summarization on Claude using a chunk size of 80,000. On average, the books are divided into 2-3 chunks. Compared to the GPT-4 summaries, these Claude summaries were considerably more readable, as they included fewer details. However, when attempting to generate span-question annotations with Claude, results were inconsistent. Sometimes, the system identified "No spans of confusion," while at other times it provided a list of annotations. As we currently do not have access to Claude's API and the playground offers no configurable parameters, we concluded that more experiments would be unnecessary.


==> sections/question-answering.tex <==
\section{Question answering} \label{sec:question-answering}

We asked GPT-4 to answer the generated questions by iterating through the book once more. The prompt can be found in Section \ref{prompt:question-answering}. However, the model would leave most of the answer areas blank, and would sometimes removing a found answer without providing a new answer during the iteration process. As discussed in Section \ref{basic-refinement}, directly asking the model to refine the summaries given span-questions pairs may have better results than asking it to first answer the questions, then refine the summaries.


==> sections/question-generation.tex <==
\section{Question generation}\label{sec:question-generation}

As an oracle experiment, we fed summaries and human-highlighted spans into the model, then asked the model to generate corresponding questions for each span. We tried it in two configurations.

\subsection{All-label question generation (2-shot)}\label{sec:all-label-question-generation}

For each book, we provide the summary and all human-highlighted spans to the model, and ask it to generate questions for all spans. In the prompt, we include the definitions of all 8 error types, and pick two books with the most human annotations as demonstrations (summary + spans + questions). The prompt can be found in Section \ref{prompt:all-label-question-generation}.

Figure \ref{fig:all-label-question-generation} shows the cosine similarity between model and human questions given the same spans. Cosine similarity was computed using the SentenceTransformers Library \footnote{https://github.com/UKPLab/sentence-transformers}. We chose the \emph{all-mp-net-based-v2} model to compute embeddings because the model has shown good performance on 14 sentence embedding datasets while being relatively fast (2800 sentences / second on a V100 GPU).

\begin{figure}[t]
\includegraphics[scale=0.5]{plots/generate-questions-cos-sims.png}
\caption{\textbf{All-label question generation}: distribution of the cosine similarity between model-generated questions and human questions}
\centering
\label{fig:all-label-question-generation}
\end{figure}

\subsection{Label-specific question generation (3-shot)}\label{sec:label-specific-question-generation}

For each book, we provide the summary and all human-highlighted spans of one error type $e$ to the model, then ask it to generate questions of type $e$ for these spans. In the prompt, we include the definition of type $e$, and pick three books with the most human annotations of type $e$ as demonstrations (summary + spans + questions). Note that we can perform 3-shot experiments in this label-specific setting because the length of each demonstration is now significantly shorter. The prompt can be found in Section \ref{prompt:label-specific-question-generation}.

The average cosine similarity for each error type is shown in Table \ref{table:label-specific-questions-generation}. Upon manual inspection, we found that model questions generally align well with human questions for all error types except language. The lower cosine similarity scores for some error types are a result of the fact that GPT-4 typically generates questions in more detail, but most of the questions are asking about essentially the same things as the human questions. This is because language errors are very subjective in our setting. An annotator may find some wording or phrasing to be slightly confusing, but other people may not consider that an issue at all.

\begin{table}[t]
\begin{tabular}{|c|c|}
\hline
\textbf{Label}  & \textbf{Avg cos sim} \\ \hline
entity omission & 0.6547               \\ \hline
event omission  & 0.5909               \\ \hline
causal omission & 0.7003               \\ \hline
salience        & 0.5715               \\ \hline
discontinuity   & 0.4930               \\ \hline
duplication     & 0.4102               \\ \hline
inconsistency   & 0.6343               \\ \hline
language        & 0.4275               \\ \hline
\end{tabular}
\centering
\caption{\textbf{Label-specific question generation}: Average cosine similarity between human questions and model questions.}
\label{table:label-specific-questions-generation}
\end{table}


==> sections/self-refine.tex <==
\section{Identify points of confusion and refine summaries} \label{basic-refinement}\label{sec:self-refine}

We asked the model to identify all points of confusion within summaries and ask corresponding questions.  then asked GPT-4 to refine these summaries with its own annotations. Both prompts can be found in Section \ref{prompt:self-refine}.

The returned spans and questions during the annotation phase were almost all related to omissions. However, demonstrations in the prompt only included span-question pairs but not full summaries. During the refinement phase, the model was able to add information into the summaries, but since the error type coverage is so low in the model annotations, the refinement task became quite trivial. 

However, the model's ability to effectively refine the summaries to some extent motivates us to run a similar experiment again with a better prompt. Section \ref{sec:question-answering} addresses issues we encountered when we asked the model to first answer the generated questions before performing any refinement. The model did a terrible job at answering questions, but the current section suggests that directly asking the model to refine the summaries may produce better results.


==> sections/source-attribution.tex <==
\section{Source attribution}\label{sec:source-attribution}

We further tested GPT-4's ability to attribute sentences in the summary to sentences in the source text. The prompt can be found in Section \ref{prompt:source-attribution}. The results had pretty high precision, but low recall (many sentences didn't get any assigned source sentences). We didn't pursue this further since from our observations, these summaries don't involve any faithfulness issues. \textcolor{red}{We should probably demonstrate this more systematically in the paper.}


==> sections/span-question-generation.tex <==
\section{Generating spans and questions}\label{sec:span-question-generation}

In this set of experiments, we only gave the model summaries, then asked it to provide both the spans and the questions. We tried it in two configurations.

\subsection{All-label span-question generation (2-shot)}\label{sec:all-label-span-question-generation}

For each book, we provide the summary and ask the model to generate a list of span-question pairs. In the prompt, we include the definitions of all 8 error types, and pick two books with the most human annotations as demonstrations (summary + spans + questions). The prompt can be found in Section \ref{prompt:all-label-span-question-generation}.

We qualitatively examined the model-generated annotations and found out that the questions are almost always related to omissions. Many questions are also answerable by the summary itself.

\subsection{Label-specific span-question generation (3-shot)}\label{sec:label-specific-span-question-generation}

For each book, we provide the summary and ask the model to generate a list of span-question pairs of a specific error type $e$. In the prompt, we include the definition of type $e$, and pick three books with the most human annotations of type $e$ as demonstrations (summary + spans + questions). The prompt can be found in Section \ref{prompt:label-specific-span-question-generation}.

Precision and recall was computed using cosine similarity. The logic is as follows:

\begin{enumerate}
    \item For each book, compute pairwise cosine similarity between all model and annotations of the given error type.
    \item For each instance in model annotations, choose the human instance with the highest cosine similarity to form a model-human pair. If the score is higher than 0.68, we consider them as a match. We compute precision using: $$\frac{\textnormal{\# of matches}}{\textnormal{\# of model annotation instances}}$$
    \item For each instance in human annotations, choose the model instance with the highest cosine similarity to form a human-model pair. If the score is higher than 0.68, we consider them as a match. We compute recall using: $$\frac{\textnormal{\# of matches}}{\textnormal{\# of human annotation instances}}$$
\end{enumerate}

The threshold for cosine similarity was established through a manual comparison of model annotations and human annotations. We discovered that a threshold of 0.68 effectively differentiates whether two annotation entries are highlighting the same issues.

Table \ref{table-label-specific-span-question-generation} shows the average precision and recall of model-generated span-question pairs. We computed numbers for three settings:

\begin{enumerate}
    \item Span-question comparison: Concatenate spans and questions together, the compare human and model annotations.
    \item Span comparison: Compare spans only.
    \item Question comparisoin: Compare questions only.
\end{enumerate}

Overall, the alignment between model and human annotations are very low. An alternative is to measure precision and recall by examining the overlap of span positions in the summaries, we will try this next.

\begin{table*}[p]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|l|l|l|l|l|}
\hline
\textbf{Label} & \textbf{All precision} & \textbf{All recall} & \textbf{Span precision} & \textbf{Span recall} & \textbf{Question precision} & \textbf{Question recall} \\ \hline
entity omission & 0.1717 & 0.1732 & 0.2535 & 0.2654 & 0.1205 & 0.1201 \\ \hline
event omission  & 0.0618 & 0.1696 & 0.1081 & 0.2807 & 0.0502 & 0.152  \\ \hline
causal omission & 0.0625 & 0.2101 & 0.0938 & 0.2521 & 0.0673 & 0.2101 \\ \hline
salience        & 0.0914 & 0.3077 & 0.1029 & 0.3654 & 0.0343 & 0.1154 \\ \hline
discontinuity   & 0.038  & 0.092  & 0.1519 & 0.3793 & 0.0084 & 0.0345 \\ \hline
duplication     & 0.27   & 0.3571 & 0.42   & 0.4762 & 0.2    & 0.2262 \\ \hline
inconsistency   & 0.1429 & 0.2967 & 0.1905 & 0.3667 & 0.1111 & 0.1667 \\ \hline
language        & 0.0189 & 0.0625 & 0.0660 & 0.1875 & 0      & 0      \\ \hline
\end{tabular}%
}
\caption{\textbf{Label-specific span-question generation}: Average precision and recall computed for all error types. Columns with the prefix "all" represent scenarios where spans and questions are concatenated and compared together. Columns with the prefix "span" represent scenarios where only the spans are compared. Columns with the prefix "question" represent scenarios where only the questions are compared.}
\label{table-label-specific-span-question-generation}
\end{table*}


==> sections/squality.tex <==
\section{SQuALITY}

\kyle{can start w/ a sentence or two of what's the objective of these SQuality experiments? why are they valuable to perform in this paper about extremely long texts?}

\reskyle{This section was included because I was trying to document everything we have done so far. The SQuALITY experiments were started before we had access to GPT-4. They were more like a playground for us to experiment with the incremental summary approach on GPT-3.5. I'm not sure if we should include this in the actual paper.}
\kyle{gotchaa; hmm, there may be a way to use them, need to think a bit more. For eample: Experimenting different iterative/hierarchical/etc. prompting workflows on Squality shows in \S\ref{sec:squality-baseline} that, if you can fit the full doc in whole context, one-pass is better than prompting workflows. Why? This makes me wonder why this is happening, and whether this is the same type of issues as being observed in our new book set? In fact, is there a common analysis around trying to build up an understanding of why errors are happening that involves a common analysis of Squality, BookSum, and this new set?}

We started with GPT-3.5 (davinci-003, now deprecated) and collected summaries on the SQuALITY dataset. Documents in the dataset have an average length of 5199.4 tokens. The context limit of the model is 4096 tokens. We settled on chunk size = 256, summary temperature = 0.1, trimming temperature = 0.5, and summary-to-story ratio = 0.15. Note that the summary-to-story ratio merely sets the maximum length for the summary, not the exact length. It does not guarantee that every summary will be 15\% of the total story length.

\reskyle{We tried two configurations for generating intermediate summaries: timeline and prose. In the timeline setting, we generated a timeline of major events at each chunk, then aggregate the final timeline into a textual summary. In the prose setting, we simply generated a textual summary at each chunk. We tried using timelines because we hypothesized that structural information might help the model keep better track of what has happened so far in the story. However, our qualitative analysis revealed that the timeline approach did not result in any improvement in summary quality.} We eventually decided to stick with prose \kyle{what's this mean?} since the timeline approach requires an extra timeline-to-prose step, and it doesn't help produce summaries of better quality.

For GPT-4, we used summary temperature = 0.5, trimming temperature = 1, summary-to-story ratio = 0.15. Note that GPT-4's temperature range is $[0, 2]$. GPT-4 produced summaries of much higher quality than GPT-3.5 in terms of coherence and readability. Since GPT-4 has a longer context window of 8192 tokens, its good performance motivated us to try it on even longer text as discussed in Section \ref{sec:book-dataset}.

\subsection{Comparison with one-pass baseline summaries}\label{sec:squality-baseline}

To study the effect of our incremental approach on the quality of the summaries, we generated SQuALITY baseline summaries by passing as much story text as possible into the model and generating a single summary. We ran our experiments on the SQuALITY dev set. Both incremental and baseline summaries were generated with temperature = 0.5, summary-to-story ratio = 0.05. For incremental summaries, we used a chunk size of 512. The prompt used for generating baseline summaries can be found in Section \ref{prompt:squality-baseline}.

Baseline summaries are generally more readable due to their lower granularity levels. Both baseline and incremental summaries can convey a story efficiently at a sensible pace. However, if the entire narrative cannot fit into the context window, baseline summaries will miss important information towards the ending of a story.

